Radio Localization and Sensing -- Part I: Fundamentals

This letter is part of a two-letter tutorial on radio localization and sensing, with focus on mobile radio systems in 5G mmWave and beyond. Part I introduces the fundamentals, covering an overview of the relevant literature, as well as the different aspects of localization and sensing problems. Then, different performance metrics are presented, which are important in the evaluation of methods. Methods are detailed in the last part of this letter. Part I thus provides the necessary background to delve into more forward-looking problems in Part II.

==> part I/acronyms.tex <==
\begin{acronym}[ACRONYM]
\acro{AI}{artificial intelligence}
\acro{AoA}{angle-of-arrival}
\acro{AoD}{angle-of-departure}
\acro{BS}{base station}
\acro{BP}{belief propagation}
\acro{CDF}{cumulative density function}
\acro{CFO}{carrier frequency offset}
\acro{CRB}{Cram\'er-Rao bound}
\acro{DA}{data association}
\acro{D-MIMO}{distributed multiple-input multiple-output}
\acro{DL}{downlink}
\acro{EM}{electromagnetic}
\acro{FIM}{Fisher information matrix}
\acro{GDOP}{geometric dilution of precision}
\acro{GNSS}{global navigation satellite system}
\acro{GPS}{global positioning system}
\acro{IP}{incidence point}
\acro{IQ}{in-phase and quadrature}
\acro{ISAC}{integrated sensing and communication}
\acro{ICI}{inter-carrier interference}
\acro{JCS}{Joint Communication and Sensing}
\acro{JRC}{joint radar and communication}
\acro{JRC2LS}{joint radar communication, computation, localization, and sensing}
\acro{IMU}{inertial measurement unit}
\acro{IOO}{indoor open office}
\acro{IoT}{Internet of Things}
\acro{IRN}{infrastructure reference node}
\acro{KPI}{key performance indicator}
\acro{LoS}{line-of-sight}
\acro{LS}{least-squares}
\acro{MCRB}{misspecified Cram\'er-Rao bound}
\acro{MIMO}{multiple-input multiple-output}
\acro{ML}{maximum likelihood}
\acro{mmWave}{millimeter-wave}
\acro{NLoS}{non-line-of-sight}
\acro{NR}{new radio}
\acro{OFDM}{orthogonal frequency-division multiplexing}
\acro{OTFS}{orthogonal time-frequency-space}
\acro{OEB}{orientation error bound}
\acro{PEB}{position error bound}
\acro{VEB}{velocity error bound}
\acro{PRS}{positioning reference signal}
\acro{QoS}{Quality of Service}
\acro{RAN}{radio access network}
\acro{RAT}{radio access technology}
\acro{RCS}{radar cross section}
\acro{RedCap}{reduced capacity}
\acro{RF}{radio frequency}
\acro{RIS}{reconfigurable intelligent surface}
\acro{RFS}{random finite set}
\acro{RMSE}{root mean squared error}
\acro{RTK}{real-time kinematic}
\acro{RTT}{round-trip-time}
\acro{SLAM}{simultaneous localization and mapping}
\acro{SLAT}{simultaneous localization and tracking}
\acro{SNR}{signal-to-noise ratio}
\acro{ToA}{time-of-arrival}
\acro{TDoA}{time-difference-of-arrival}
\acro{TR}{time-reversal}
\acro{TXRX}[TX/RX]{transmitter/receiver}
\acro{Tx}{transmitter}
\acro{Rx}{receiver}
\acro{UE}{user equipment}
\acro{UL}{uplink}
\acro{UWB}{ultra wideband}
\acro{XL-MIMO}{extra-large MIMO}
\end{acronym}

==> part I/authors.tex <==
\author{Henk Wymeersch,~\IEEEmembership{Senior Member,~IEEE}, 
        Gonzalo Seco-Granados,~\IEEEmembership{Senior Member,~IEEE}
\thanks{
This work was supported by the European Commission through the H2020 project Hexa-X (Grant Agreement no.~101015956),by the ICREA Academia Program, and by the Spanish R+D project PID2020-118984GB-I00.}
\thanks{Henk Wymeersch is with the Department
of Electrical Engineering, Chalmers University of Technology, 41258 Gothenburg, Sweden (e-mail: henkw@chalmers.se). %}
%\thanks{
Gonzalo Seco-Granados is with the Department of Telecommunications and Systems Engineering, Universitat Autonoma de Barcelona, 08193 Bellaterra, Barcelona, Spain (e-mail: gonzalo.seco@uab.cat).}}


==> part I/commands.tex <==
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newcommand{\el}{(\mathrm{el})}
\newcommand{\az}{(\mathrm{az})}
\newcommand{\BS}{\mathrm{BS}}
\newcommand{\UE}{\mathrm{UE}}
\newcommand{\SP}{\mathrm{SP}}
\newcommand{\A}{\mathrm{A}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\vecR}{\mathbf{r}}
\newcommand{\bnot}[1]{\boldsymbol{#1}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\Transpose}{^\top}
\newcommand{\Hermitian}{^\mathrm{H}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\vect}{\mathrm{vec}}
\newcommand{\CRB}{^{(\mathrm{CRB})}}
\newcommand{\CCRB}{^{(\mathrm{CCRB})}}
\newcommand{\acos}{\mathrm{acos}}
\newcommand{\atan}{\mathrm{atan}}
\makeatletter
\newcommand{\gettikzxy}[3]{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}
\definecolor{mygray}{gray}{0.6}
\newcommand{\todo}[1]{\textcolor{mygray}{\footnotesize{\textsf {[ #1]}}}}
\newcommand{\rev}[1]{\textcolor{blue}{#1}}

==> part I/figures/FiguresPartI/letterPartI.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor2}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor3}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor4}{rgb}{0.30100,0.74500,0.93300}%
%

\begin{tikzpicture}[scale=1\columnwidth/10cm,font=\footnotesize]
\begin{axis}[%
width=8cm,
height=4cm,
%at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1,
xmax=122.88,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Bandwidth [MHz]},
ymode=log,
ymin=0.001,
ymax=1000,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={RMSE of first object [m]},
axis background/.style={fill=white},
 legend columns=3, 
%legend style={legend cell align=left, align=left, draw=white!15!black}
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(-0.01, 0.05)},
  align=left,
  legend cell align=left,
  anchor=south west
%  draw=white!80!black
}
]
\addplot [color=red, dashed, line width=2.0pt,mark=*]
  table[row sep=crcr]{%
0.96	10.1509694172485\\
1.92	5.14970161832234\\
3.84	2.5408092751538\\
7.68	1.30674528931586\\
15.36	0.652093111554356\\
30.72	0.340189886532389\\
61.44	0.164912997200748\\
122.88	0.0802661635651633\\
};
\addlegendentry{RMSE (1 path)}

\addplot [color=blue, dashed, line width=2.0pt]
  table[row sep=crcr]{%
0.96	58.763017051396\\
1.92	46.1427504108384\\
3.84	38.7833344095675\\
7.68	29.706074064325\\
15.36	7.57583824994693\\
30.72	0.8822787811436\\
61.44	0.22034914153635\\
122.88	0.0900872668620709\\
};
\addlegendentry{RMSE (5 paths)}

\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
0.96	312.5\\
1.92	156.25\\
3.84	78.125\\
7.68	39.0625\\
15.36	19.53125\\
30.72	9.765625\\
61.44	4.8828125\\
122.88	2.44140625\\
};
\addlegendentry{resolution}

\addplot [color=black, line width=1.0pt]
  table[row sep=crcr]{%
0.96	20\\
1.92	20\\
3.84	20\\
7.68	20\\
15.36	20\\
30.72	20\\
61.44	20\\
122.88	20\\
};
\addlegendentry{inter-path distance}

\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
0.96	10.9827344826809\\
1.92	5.45896951173931\\
3.84	2.72547964035069\\
7.68	1.36224055662308\\
15.36	0.68105791322618\\
30.72	0.340521162315681\\
61.44	0.170259606912477\\
122.88	0.0851296816768743\\
};
\addlegendentry{CRB (1 path)}

\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
0.96	14611590.9303994\\
1.92	3759809.28196941\\
3.84	24833.2707559492\\
7.68	229.619157136688\\
15.36	2.89520309818785\\
30.72	0.364853998550178\\
61.44	0.172989796619058\\
122.88	0.0854820728286714\\
};
\addlegendentry{CRB (5 paths)}

\end{axis}

\end{tikzpicture}%

==> part I/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{bm}
\usepackage{epsfig,amsfonts,amsbsy,bm,mathrsfs}
\usepackage{amssymb,amsmath,amsthm,latexsym,amscd,amsfonts}
\usepackage{lettrine}
\usepackage{authblk}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag,float}
\usepackage{pstricks}
\usepackage{pst-plot}
% \usepackage{caption}
% \usepackage{subcaption}
\usepackage{cite}
\usepackage{balance}
\usepackage{epsfig}
\usepackage{epstopdf}
\usepackage{bbm}
\usepackage{enumitem}
\usepackage{dsfont}
\usepackage{setspace}
\usepackage{float}
\usepackage{relsize}
\usepackage{comment}
\usepackage{subfigure} % For subfigures
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
%\usepackage{hyperref}
\usepackage[nolist]{acronym}
%\usepackage[table]{xcolor}
\usepackage{tabularx}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{units}

\usepackage{tikz}
\usetikzlibrary{calc}
%\usepackage{arydshln}
\usepackage{xcolor}
\usepackage{tabularx}
\usepackage{colortbl}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{plotmarks}
\usetikzlibrary{arrows.meta}
\usepgfplotslibrary{patchplots}
\usepackage{grffile}
\newlength\fheight 
\newlength\fwidth 
\usepgfplotslibrary{fillbetween}

